An Image Segmentation Model Based on a Variational Formulation

Starting from a variational formulation, we present a model for image segmentation that employs both region statistics and edge information. This combination allows for improved flexibility, making the proposed model suitable to process a wider class of images than purely region-based and edge-based models. We perform several simulations with real images that attest to the versatility of the model. We also show another set of experiments on images with certain pathologies that suggest opportunities for improvement.

==> bimodal.tex <==
\begin{figure}
\centering
	\begin{tikzpicture}
	\begin{scope}[blend group = soft light]
	\draw[blue!60!white,thick]   ( 90:1.2) circle (2);
	\fill[red!30!white]   ( 90:1.2) circle (2);
	\end{scope}
	\node at ( 90:2)    {Foreground};
	\node at ( 330:2)   {Background};
	\node[font=\Large] at (3,1.8) {$ \omega $};
	\draw[->, thick] (3,1.5) -- (2,1);
	 \draw [very thick, rounded corners, dashed] (-3,2) to[out=45,in=115] (-1,1) to[out=-180+115,in=10] (-3,-1) to [out=190,in=45+180](-3,2);
	 \node[font=\large] at (-4.2,1.5) {$C(\X,t)  $};
		\end{tikzpicture} \caption[Composition of a bimodal image.]{Composition of a bimodal image. Foreground (in color), background, and the boundary $ \omega $ (in blue) separating the two regions. A segmentation is obtained as $ C $  approaches $ \omega $.}
		\label{composition} \end{figure}

==> cornerneighbors.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=.75]
\draw [help lines] (0,0) grid (4,-4);%grid
%axes
\draw[thick,->] (0,0)--(0,-5) node[anchor=east] {\large $x$};	%vertical axis
\draw[thick,->] (0,0)--(5,0) node[anchor=west] {\large $y$};	%horizontal axis
%interior pixels
\foreach \x in {1,2,3}
	\foreach \y in {-3,-2,-1}
		\draw  (\x,\y) circle (5pt);;
\filldraw (7,-2) circle (5pt) node[anchor=west] {\large \quad pixel $ (i,j) $};	
\filldraw[gray] (7,-3) circle (5pt); \node[right] at (7,-3) {\large \quad corner neighbors };	\filldraw[black] (2,-2) circle (5pt); 
\filldraw[gray] (1,-1) circle (5pt);
\filldraw[gray] (1,-3) circle (5pt);
\filldraw[gray] (3,-1) circle (5pt);
\filldraw[gray] (3,-3) circle (5pt);
%x labels
\node[anchor= east] at (0,-1) {$ i-1 $};
\node[anchor= east] at (0,-2) {$ i $};
\node[anchor= east] at (0,-3) {$ i+1 $};
%j labels
\node[anchor= south] at (1,0) {\small $ j-1 $};
\node[anchor= south] at (2,0) {$ j $};
\node[anchor= south] at (3,0) {\small $ j+1 $};
\end{tikzpicture} 
\caption[$ 3 \times 3 $ neighborhood of pixel $(i,j)  $.]{$ 3 \times 3 $ neighborhood of pixel $(i,j)  $. Corner neighbors are used for approximating mixed second order derivatives.}
\label{fig:neighbors}
\end{figure}


==> galaxyexample.tex <==
\begin{figure}
\centering
\subfloat[]{%
\resizebox*{.23\linewidth}{!}{	\includegraphics[width=\textwidth]{galaxy}}}
\subfloat[]{%
\resizebox*{.23\linewidth}{!}{	\includegraphics[width=\textwidth]{galaxy_inic}}}
\subfloat[]{%
\resizebox*{.23\linewidth}{!}{\includegraphics[width=\textwidth]{galaxy_finalMS}}}
\subfloat[]{%
\resizebox*{.23\linewidth}{!}{\includegraphics[width=\textwidth]{galaxy_finalEMS}}}
	\caption[A successful segmentation of `galaxy' image by our proposed model.]{A successful segmentation of `galaxy' image by our proposed model. The ``congnitive" boundary of the galaxy is suggested by our model. (a) Orignal image; (b) initial curve; (c) Result with MS model; (d) result with proposed EMS model.}
 	\label{im:galaxy}
\end{figure}

==> inictests.tex <==
\begin{figure}
\centering
%a
\subfloat[]{\label{correct1}
\resizebox*{.45\linewidth}{!}{
    \includegraphics[width=.5\textwidth]{twocells_ini}%
    \includegraphics[width=.5\textwidth]{twocells_good}}}
\subfloat[]{%b
\resizebox*{.45\linewidth}{!}{	\includegraphics[width=.5\textwidth]{middlerect_ini}%    
 		\includegraphics[width=.5\textwidth]{middlerect_final}}}\\
%c 		
\subfloat[]{
\resizebox*{.45\linewidth}{!}{	\includegraphics[width=.5\textwidth]{rightellipse_inic}%    
 		\includegraphics[width=.5\textwidth]{rightellipse_final}}}
 		\subfloat[]{
\resizebox*{.45\linewidth}{!}{	\includegraphics[width=.5\textwidth]{leftellipse_inic}%    
 		\includegraphics[width=.5\textwidth]{leftellipse_final}}}\\
 		\subfloat[]{\label{correct2}
\resizebox*{.45\linewidth}{!}{	\includegraphics[width=.5\textwidth]{twocells_2elli_ini}%    
 		\includegraphics[width=.5\textwidth]{twocells_2elli_final}}}
 		\subfloat[]{
\resizebox*{.45\linewidth}{!}{	\includegraphics[width=.5\textwidth]{twocells_topleft_ini}%    
 		\includegraphics[width=.5\textwidth]{twocells_topleft_final}}}\\
 		\subfloat[]{
\resizebox*{.45\linewidth}{!}{	\includegraphics[width=.5\textwidth]{tcellsbcrini}%    
 		\includegraphics[width=.5\textwidth]{twocells_bottomcenter_final}}}
 		\subfloat[]{\label{correct3}
\resizebox*{.45\linewidth}{!}{	\includegraphics[width=.5\textwidth]{twocells_all_ini}%    
 		\includegraphics[width=.5\textwidth]{twocells_all_final}}}\\

			 \caption[Sensitivity to initialization for the proposed variational model.]{Sensible initialization of the evolving front plays a crucial role in the segmentation results for the proposed model.  When initial contours encompass the target objects, as in \sref{correct1} and \sref{correct2}, meaningful results are obtained. In \sref{correct3} an almost correct segmentation is obtained if the detected region inside the cell on the left is neglected.}
 			\label{im:inicondexperiments}
\end{figure}


==> monkeyexample.tex <==
\begin{figure}
\centering
\subfloat[Original image and initial curve.]{%
\resizebox*{5cm}{!}{\includegraphics{monkey_ini.png}}}\hspace{5pt}
\subfloat[Final segmentation.]{%
\resizebox*{5cm}{!}{\includegraphics{monkey_badseg.png}}}
\caption[Incorrect segmentation using Separation of Means.]{Incorrect segmentation using separation of means. The evolving curve is attracted to the brightest regions in the image.}
	\label{monkeymeansep}
\end{figure}

==> monkeyexample2.tex <==
\begin{figure}
\centering
\subfloat[]{%
\resizebox*{.3\linewidth}{!}{\includegraphics{monkey_inibw}}}
\subfloat[]{%
\resizebox*{.3\linewidth}{!}{\includegraphics{monkey_badsegbw.png}}}
\subfloat[]{%
\resizebox*{.3\linewidth}{!}{\includegraphics{monkey_goodsegbw}}}
\caption[Successful segmentation of `monkey' image by our proposed model.]{Successful segmentation using our proposed model. (a) Image and initial curve; (b) result with the MS model; (c) result with the proposed EMS model.}
	\label{monkeygoodseg}
\end{figure}

==> noisy.tex <==
\begin{figure}[!htbp]
%file: noisy.tex
\centering
	\includegraphics[width=.45\textwidth]{nini}\includegraphics[width=.45\textwidth]{nfinal}
		\caption[Effect of noise.]{Effect of noise. Noise removal techniques ought to be implemented before segmentation.}
		\label{fig:noise}
\end{figure}

% noisy_ini   ~ nini
% noisy_final ~ nfinal


==> trimodal1.tex <==
\begin{figure}
\centering
\subfloat[]{
\resizebox*{.45\linewidth}{!}{
    \includegraphics[width=\textwidth]{trimodal1_ini}}}
\subfloat[]{\label{}
\resizebox*{.45\linewidth}{!}{
    \includegraphics[width=\textwidth]{trimodal1_final}}} 
			\caption[Segmentation of trimodal image with triple junction.]{Segmentation of trimodal image with triple junction. (a) Original image and initial curve; (b) result by proposed model. Boundaries of the outer square are detected.}
	\label{im:trimodal}
\end{figure}


==> trimodalb.tex <==
\begin{figure}
\centering
\subfloat[]{\label{fig:black2}
\resizebox*{\linewidth}{!}{
    \includegraphics[width=\textwidth]{bwsq_black_ini}\includegraphics[width=\textwidth]{bwsq_black_final}}}\\
    \subfloat[]{\label{fig:white2}
\resizebox*{\linewidth}{!}{
    \includegraphics[width=\textwidth]{bwsq_white_ini}\includegraphics[width=\textwidth]{bwsq_white_final}}} 
    \caption[Selective segmentation in trimodal image with triple junction.]{Selective segmentation in trimodal image with triple junction. Individual detection of \sref{fig:black2} black and \sref{fig:white2} white rectangle.}
 	\label{im:trimodal1}
\end{figure}


==> trimodalsep.tex <==
\begin{figure}[!htbp]
\centering
\centering
\subfloat[]{\label{fig:wh11f}
\resizebox*{.9\linewidth}{!}{
    	\includegraphics[width=.5\textwidth]{bwsq_sepw_ini}
    	\includegraphics[width=.5\textwidth]{bwsq_sepw_final}}}\\
    \subfloat[]{\label{fig:white32}
\resizebox*{.9\linewidth}{!}{
    	\includegraphics[width=.5\textwidth]{bwsq_sepb_ini}
    	\includegraphics[width=.5\textwidth]{bwsq_sepb_final}}} 
		\caption[Segmentation of image with 4 regions]{\sref{fig:wh11f} Selective detection is still possible, \sref{fig:white32} but detection of all objects in the scene is not.}
	\label{im:trimodal2}
\end{figure}

==> twocellsexample.tex <==
\begin{figure}
\centering
\subfloat[]{%
\resizebox*{.23\linewidth}{!}{	\includegraphics[width=\textwidth]{twocells}}}
\subfloat[]{%
\resizebox*{.23\linewidth}{!}{	\includegraphics[width=\textwidth]{twocells_ini}}}
\subfloat[]{%
\resizebox*{.23\linewidth}{!}{\includegraphics[width=\textwidth]{twocells_bad}}}
\subfloat[]{%
\resizebox*{.23\linewidth}{!}{\includegraphics[width=\textwidth]{twocells_good}}}
		\caption[Segmentation results for `two cells' image.]{(a) Original image and (b) initial curve; (c) results with the MS model and (d) the proposed EMS model. The two cells are successfully detected by our model.}
 \label{im:twocells}
\end{figure}
